Federated Momentum Contrastive Clustering

We present federated momentum contrastive clustering (FedMCC), a learning framework that can not only extract discriminative representations over distributed local data but also perform data clustering. In FedMCC, a transformed data pair passes through both the online and target networks, resulting in four representations over which the losses are determined. The resulting high-quality representations generated by FedMCC can outperform several existing self-supervised learning methods for linear evaluation and semi-supervised learning tasks. FedMCC can easily be adapted to ordinary centralized clustering through what we call momentum contrastive clustering (MCC). We show that MCC achieves state-of-the-art clustering accuracy results in certain datasets such as STL-10 and ImageNet-10. We also present a method to reduce the memory footprint of our clustering schemes.

==> 035-memefficient.tex <==
\section{Memory-Efficient MCC and FedMCC}
\label{secmemefficient}
An important special case of the federated learning paradigm is when the clients are low-cost edge devices that may have memory limitations. The amount of training memory needed for a naive implementation of the gradient descent updates for the loss function in (\ref{mcclossfunc}) or its federated counterparts in (\ref{eq:fed_Lins}) and (\ref{eq:fed_Lclu}) is linear in the batch size $n$. For the example case of the CC, this is because the network outputs $\{z_i^{\sigma,\nu}, y_i^{\sigma,\nu}\},\,i=1,\ldots,n$ for different members of a batch $x_i,\,i=1,\ldots,n$ are coupled in a non-linear manner in the loss functions. Hence, to perform a gradient update, the size of the computation graph should be roughly of size $n\eta$, where $\eta$ represents the neural network size. This is in contrast to ordinary batch loss of the form $\sum_{i=1}^n \ell(x_i)$, where $x_i$ are inputs and $\ell$ is some loss function. In this case, the gradient of the entire loss function can be calculated through accumulation using only one computation graph of size $\eta$.

%$\theta$ represents the parameters of the size-$\eta$ neural network, 

Our idea for constructing memory-efficient MCC and FedMCC is akin to the scheme presented in \cite{gao2021scaling} for the case of ordinary contrastive learning. We first calculate the gradients of the loss function with respect to the network outputs or representations. These gradients are calculated over one pass over the batch and stored on the memory. The memory overhead of this first stage is relatively low as the dimensionality of representation vectors is much smaller than that of the parameter space. A second pass over the batch can then update the network parameters. Due to space limitations, we describe the details of the procedure in the supplemental material. 

% To describe the details of this procedure, let us now extend the CC scheme to a memory-efficient CC scheme. Extensions to MCC and FedMCC can be accomplished in the same fashion and will thus be omitted for brevity.

% We recall the loss function for the CC scheme in (\ref{lccloss}). The goal is to calculate the gradient $\frac{\partial L_{CC}}{\partial \theta}$, where $\theta$ represents the neural network parameters. For each $i\in\{1,\ldots,n\}$, let us define the gradients
% \begin{align}
% \label{alphas123} \alpha_{i,1} \triangleq \frac{1}{2}\frac{\partial L(\mathbf{z}^a, \mathbf{z}^b; \tau_I)}{\partial z_i^a}, \alpha_{i,2} \triangleq \frac{1}{2}\frac{\partial L(\mathbf{z}^a, \mathbf{z}^b; \tau_I)}{\partial z_i^b},  \alpha_{i,3} \triangleq \frac{1}{2}\frac{\partial L(\mathbf{c}^a, \mathbf{c}^b; \tau_C)}{\partial y_i^a}, \\ \label{alphas456} \alpha_{i,4} \triangleq \frac{1}{2}\frac{\partial L(\mathbf{c}^a, \mathbf{c}^b; \tau_C)}{\partial y_i^b},
%  \alpha_{i,5} \triangleq \frac{\partial H(\mathbf{c}^a)}{\partial y_i^a}, \alpha_{i,6} \triangleq \frac{\partial H(\mathbf{c}^b)}{\partial y_i^b}.
% \end{align}
% The partial derivative of the overall loss function with respect to one of the parameters $\theta'\in\theta$ is then expressed as 
% \begin{multline}
% \label{lccform1}
% \frac{\partial L_{CC}}{\partial \theta} = \sum_{i=1}^n \Bigl[ \Bigl\langle \alpha_{i,1},\frac{\partial z_i^a}{\partial \theta'}\Bigr\rangle + \Bigl\langle \alpha_{i,2},\frac{\partial z_i^b}{\partial \theta'}\Bigr\rangle + \\ \Bigl\langle \alpha_{i,3} \!+\! \alpha_{i,5},\frac{\partial y_i^a}{\partial \theta'}\Bigr\rangle \!+\! \Bigl\langle \alpha_{i,4}\!+\!\alpha_{i,6},\frac{\partial y_i^b}{\partial \theta'}\Bigr\rangle \Bigl].
% \end{multline}
% Note that, for any input index $i\in\{1,\ldots,n\}$ in a batch, the gradients $\frac{\partial z_i^{\sigma}}{\partial \theta'},\,\frac{\partial y_i^{\sigma}}{\partial \theta'},\,\sigma\in\{a,b\}$ in (\ref{lccform1}) depend only on $x_i$ (and are independent of $x_j,\,j\neq i$). Hence, if $\alpha_{i,j},\,i\in\{1,\ldots,n\},\,j\in\{1,\ldots,6\}$ are known, or calculated beforehand, the entire partial derivative (\ref{lccform1}) assumes the form of an ``ordinary batch loss'' $\sum_{i=1}^n \ell(x_i)$, as described in the beginning of this section. In fact, the parameters $\alpha_{i,j}$ can simply be calculated by a single forward pass of the entire batch (possibly one input at a time to save memory) before the gradient updates. As a result, once $\alpha_{i,j}$ are known, (\ref{lccform1}) can be calculated one input at a time through gradient accumulation. Moreover, for each given input, the standard backpropagation algorithm can be used to calculate the partial derivatives for all parameters of the network simultaneously. 

% Closed-form expressions for the gradients $\alpha_{i,j},\,i\in\{1,\ldots,n\},\,j\in\{1,\ldots,6\}$ follow from cumbersome but basic calculus. To provide the final expressions, for any $i\in\{1,\ldots,n\}$, let
% \begin{align}
% \xi_i \triangleq \sum_{\substack{j=1 \\ j \neq i}}^n \Bigl[\exp(\tfrac{1}{\tau}s(u_i,u_j)) \!+\! \exp(\tfrac{1}{\tau}s(u_i,v_j)) \Bigr],
% \end{align}
% We also define
% \begin{align}
% \label{algebra1}
% s'(u,v)\triangleq \frac{\partial s(u,v)}{\partial u} = \frac{s(u,v)}{\|u\|^2} u + \frac{1 }{\|u\|\|v\|} v,
% \end{align}
% using which we can provide the closed-form expressions
% \begin{align}
%  \nonumber n \tau  & \frac{\partial L(\mathbf{u},\mathbf{v};\tau)}{\partial u} = -s'(u_{\ell},v_{\ell})  + \\  \label{algebra2} & 
% \sum_{\substack{i=1 \\ i \neq {\ell}}}^n \Bigl[ \Bigl(\frac{1}{ \xi_{\ell}}+\frac{1}{ \xi_{i}}\Bigr) \exp(\tfrac{1}{\tau}s(u_{\ell},u_i))s'(u_{\ell},u_i) + 
% \exp(\tfrac{1}{\tau}s(u_{\ell},v_i))s'(u_{\ell},v_i)\Bigr], \\
% \label{algebra3} n \tau & \frac{\partial  L(\mathbf{u},\mathbf{v};\tau) }{\partial v}  = 
% -s'(v_{\ell},u_{\ell}) + \sum_{\substack{i=1 \\ i \neq \ell}}  \frac{1}{ \xi_i} \exp(\tfrac{1}{\tau}s(v_{\ell},u_{i}))s'(v_{\ell},u_{i})
% \end{align}
% for the gradients of $L(\mathbf{u},\mathbf{v};\tau)$. In addition, with regards to the entropies that appear in the loss function, we can evaluate, for any $\ell\in\{1,\ldots,d\}$,
% \begin{align}
% \label{algebra4}
%     \frac{\partial H(\mathbf{u})}{\partial u_{\ell}} 
%         =  \sum_{i=1}^{d} \frac{\|u_i\|_1-\mathbf{1}(i=\ell)\|\mathbf{u}\|_1}{\|\mathbf{u}\|_1^2}\left(1+\log \frac{\|u_i\|_1}{\|\mathbf{u}\|_1}\right)\mathrm{sign}(u_{\ell}).
% \end{align}
% As mentioned, formulae (\ref{algebra1})-(\ref{algebra4}) can be verified using straightforward calculations. Now, $\alpha_{i,1}$ and $\alpha_{i,2}$ in (\ref{alphas123}) can be calculated via (\ref{algebra2}). For $\alpha_{i,3}$, we can first use the identity
% \begin{align}
% \label{laksjdlaksd}
% \left[ \alpha_{1,3} \cdots \alpha_{n,3} \right] \!=\! \frac{1}{2}\left[\frac{\partial L(\mathbf{c}^a, \mathbf{c}^b; \tau_C)}{\partial c_1^a} \cdots \frac{\partial L(\mathbf{c}^a, \mathbf{c}^b; \tau_C)}{\partial c_d^a} \right]^{\dagger}\!\!\!\!,\!\!\!\!
% \end{align}
% where $c_1^{\sigma},\ldots,c_n^{\sigma}$ represent the columns of $\mathbf{c}^a$. Now, the right hand side of (\ref{laksjdlaksd}) can be calculated through (\ref{algebra3}). Likewise, $\alpha_{i,4},\alpha_{i,5}$, and $\alpha_{i,6}$ can be evaluated via (\ref{algebra2}), (\ref{algebra3}),  (\ref{algebra4}), and the transposition method in (\ref{laksjdlaksd}).

